How accurate are stellar ages based on stellar models ? I. The impact of stellar models uncertainties

Among the various methods used to age-date stars, methods based on stellar model predictions are widely used, for nearly all kind of stars in large ranges of masses, chemical compositions and evolutionary stages. The precision and accuracy on the age determination depend on both the precision and number of observational constraints, and on our ability to correctly describe the stellar interior and evolution. The imperfect input physics of stellar models as well as the uncertainties on the initial chemical composition of stars are responsible for uncertainties in the age determination. We present an overview of the calculation of stellar models and discuss the impact on age of their numerous inputs.

==> abundances.tex <==
\subsection{Chemical composition}

The initial chemical composition is, after the initial mass, the second main input of stellar models. 
It is usually expressed in mass fraction.
The abundances in mass fraction of H, He, and metals (\ie, of all elements heavier than helium) 
are denoted respectively by $X$, $Y$, and $Z$. The abundance of a given element ${i}$ is denoted by $X_{i}$. 
Since observations generally provide abundances relative to hydrogen, 
very often, the global abundance of metals is expressed by the ratio $Z/X$ (see below).

All elements do not intervene at the same level in stellar model calculation.
On one hand, some elements directly enter the calculation of the stellar structure via the physical 
processes (nuclear reaction rates, opacity, equation of state, diffusion, etc.), and thus, their abundances impact the structure of the star.
For instance,
\begin{itemize}
\item the nuclear reaction rates are dominated by H (on the MS), then by He, C, O, etc.,
\item the mean Rosseland opacity is governed by some leading elements, mainly H, He, Fe, O, Ne, etc.,
\item the equation of state requires the global amount of metals $Z$ that intervenes in the pressure calculation, 
as well as the individual abundances $X_{i}$ that intervene in the calculation of ionization equilibria,
\item the microscopic diffusion --and more generally transport processes-- concern all the elements.
\end{itemize}
On the other hand, some elements are tracers of transport processes and their abundances do not impact much the star structure 
(for instance $\ ^{6, 7}\mathrm{Li}$, $\ ^{9}\mathrm{Be}$, $\ ^{13}\mathrm{C}$, etc.).
The nature of leading elements, for a given process, depends on the physical conditions inside the star ($T$, $P$), and therefore on the mass and evolution state.

\subsubsection{Heavy elements}

Observations provide present surface abundances, not initial abundances nor inner abundances. 
In the case of the Sun, observations in the photosphere, meteorites, and interstellar medium 
provide individual abundances of all elements $X_{i}$, isotopic ratios, and the global $Z/X$ 
\citep[see \eg,][]{2009ara&a..47..481a}. Stellar data are sparser. 
Generally, one has access to the abundance in number of metals relative to hydrogen [M/H] or to [Fe/H] 
(if only iron is measured) and sometimes to a few individual abundances like those of C, N, O, Ca, or $\alpha$-elements (see below).

In the modelling, one uses the ratio $Z/X$ of abundances in mass fraction, which is related to the observed abundances in number by the following relation,
\begin{equation}
\mathrm{[M/H]}=\log (Z/X)- \log (Z/X)_\odot,
\end{equation}
where a value for the solar $(Z/X)_\odot$ has to be chosen (see below), 
and where $\mathrm{[M/H]}$ is often taken to be equal to $\mathrm{[Fe/H]}$.
One also has to choose a mixture of heavy elements, \ie,  the abundances of individual metals. Usually, it is assumed that 
$(X_{i}/Z)=(X_{i}/Z)_\odot$ unless individual abundances are measured (for instance $\alpha$-elements enhanced mixture, CNONa in globular clusters, etc.).

In the following sections, we examine the impact of the abundances of heavy elements on age. For that purpose, we consider 
as examples, the solar mixture ([Fe/H]=0), a depleted mixture with [Fe/H]=$-1.0$ dex (representative of some halo or thick disc stars), 
and an $\alpha$-elements enhanced mixture.

\subsubsection{Helium}

The helium abundance cannot be inferred directly from the spectra of tepid stars because of the lack of lines.
In the Sun, the helium abundance in the convective envelope (CE) has been inferred  from helioseismology (see Lecture 2 on \textsl{The impact of asteroseismology})).
The helioseismic solar value is $Y_\mathrm{CE, \odot}= 0.2485\pm 0.0034$ \citep{2004ApJ...606L..85B}. 
 Because of diffusion processes that occurred during the solar lifetime, $Y_\mathrm{CE, \odot}$ is expected to be different from 
 the initial helium abundance in the molecular cloud where the Sun formed. From the calibration of the solar model, \ie,  from the requirement that 
 a model of $1\ M_\odot$ reaches at solar age $t_\odot \sim 4.57$~\Gyr, the observed solar luminosity, radius, and surface metal abundance $(Z/X)_\odot$,
  one derives the solar initial helium abundance $Y_\mathrm{0, \odot}$ and metal to hydrogen ratio $(Z/X)_\mathrm{0, \odot}$. 
  The solar model calibration also provides the convection parameter $\alpha_\mathrm{conv}$ (see Sect.~\ref{conv}).
More details about the solar model calibration are given in Lecture 2 (\textsl{The impact of asteroseismology}). 
 
 The initial helium abundance $Y_0$ is therefore usually a free parameter of stellar models. 
The main hypothesis/choices that are currently made for this quantity are listed below.
\begin{itemize}
\item $Y_0$ can be set to the solar calibrated value $Y_\mathrm{0, \odot}$, which depends on the input physics of the 
associated solar model.
\item $Y_0$ can be derived from the relation $Y_0= Y_\mathrm{p} + Z\times (\Delta Y/\Delta Z)$, where $  Y_\mathrm{p} $ 
is the primordial helium abundance, and  $\Delta Y/\Delta Z$ the helium-to-heavy elements enrichment ratio.
This relation accounts for the enrichment of helium and heavy elements in the interstellar medium resulting 
from Galactic evolution. The value of the primordial helium abundance is quite secure today. 
For instance, on one hand, 
\citet{2013JCAP...11..017A} got $Y_\mathrm{p}=0.2534 \pm 0.0083 $ from observations in H\textsc{ii} regions. 
On the other hand, from the observations of the Cosmic Microwave Background by the  WMAP and 
Planck missions and standard Big Bang nucleosynthesis, \citet{2008JCAP...11..012C}  
inferred $Y_\mathrm{p}=0.2487 \pm 0.0002$ (WMAP), while \citet{2013arXiv1307.6955C} 
inferred $Y_\mathrm{p} = 0.2463 \pm 0.0003$ (Planck). 
 Conversely, $\Delta Y/\Delta Z$ is imprecise and can vary from place to place in the Galaxy.
Stellar modellers currently use values in the range $\Delta Y/\Delta Z=2 \pm 1$, resulting from solar calibration. However, 
as reported by \citet{2010A&A...518A..13G}, a large dispersion is found in the literature  with 
$\Delta Y/\Delta Z$ values that vary from $0.5$ to $5$ at least.
\item In most favourable cases, where precise and numerous observational constraints are available for the considered star, 
the initial helium content of the star can be inferred from modelling. This is \`{a} la carte modelling, 
thoroughly described in lecture 2.
\end{itemize}

In the following, to estimate the impact of the choice of $Y$ on age-dating, we consider models with 
$Y=0.25, 0.28$, and $0.31$, and  $\Delta Y/\Delta Z= 2$ and $5$.

\subsubsection{Solar mixture}
\label{solarmixture}

In most stellar models, stellar mixtures are assumed to be similar to the solar mixture, \ie,  $(X_{i}/Z)_\mathrm{star}=(X_{i}/Z)_\odot$.
However, the choice to make on the solar mixture is still subject to discussion. In the years from 1993 to now, 
there have been several revisions of the solar photospheric mixture. A major revision took place in 2003, 
when 3-D solar model atmospheres including non local thermodynamical equilibrium effects 
as well as improved atomic data were used to infer solar photospheric abundances \citep[see \eg,][]{2009ara&a..47..481a}. 
The unexpected result has been a decrease of the abundances of C, N, O, Ne, Ar, and $\left(Z/X\right)_\odot$. 
In Table~\ref{solar_global} below, we list some of the $\left(Z/X\right)_\odot$ determinations.

\begin{table}[ht]
\begin{center}
\caption{Values of the solar $\left(Z/X\right)_\odot$ ratio from 1993 to 2010 obtained successively by 
\citet{1993pavc.conf..205G} ({\small GN93}), \citet{1998SSRv...85..161G} ({\small GN98}),
\citet{2005A&A...435..339A} ({\small AGS05}), \citet{2008A&A...488.1031C} (Caff08), \citet{2009ara&a..47..481a} ({\small AGSS09}), and \citet{2009LanB...4B..712L} (Lod09). }
\label{solar_global}
\centering
\begin{tabular}{ l c c cccc}
\noalign{\smallskip}
\hline\hline
\noalign{\smallskip}
 & {\small GN93} & {\small GN98} & {\small AGS05} & Caff08 & {\small AGSS09} &	 Lod09  \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
 $\left(Z/X\right)_\odot$ & 0.0245 & 0.0229 & 0.0165& 0.0209 & 0.0181 & 0.0191  \\
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
\end{table}

From the {\small GN93} to the {\small AGSS09} results, the solar oxygen abundance decreased by $\sim 34$ per cent. 
This impacted the total solar metallicity $\left(Z/X\right)_\odot$, 
which decreased by $\sim 25$ per cent. One of the main consequences is a degradation of the agreement between the 
helioseismic solar model and observations \citep[\eg,][]{2009ara&a..47..481a}. 
The decrease of the O abundance induces a decrease of opacity, 
which leads to a convective envelope shallower than the seismically inferred value. 
The $\mu$-decrease degrades the agreement between solar model structure and helioseismology observations. 
It has been suggested that an increase of the Ne abundance (non directly measured in the solar photosphere)  
could compensate for the oxygen decrease. 
However, while the  increase in opacity due to Ne improves 
the agreement with helioseismology for the location of the base of the convective zone and the He abundance in it, 
the density and sound speed profiles still do not match the seismic estimates 
\citep[for a review, see][]{2008PhR...457..217B}.
 In the following, we consider the effects on age-dating
of a change from the {\small GN93} mixture to the {\small AGSS09} one. 

\subsubsection{$\alpha$-elements}

In stars, the $\alpha$-elements (O, Ne, Mg, Si, S, Ar, Ca, Ti) are synthesized by $\alpha$ particles (\eg, helium nuclei) capture reactions that  proceed as,
\begin{equation}
\ _{6}^{12}\mathrm{C} (\alpha, \gamma) \ _{8}^{16}\mathrm{O} (\alpha, \gamma) \ _{10}^{20}\mathrm{{Ne}} (\alpha, \gamma) \ _{12}^{24}\mathrm{{Mg}} (\alpha, \gamma)\dots
\end{equation}
and so on up to the synthesis of Si, S, Ar, Ca, and Ti. In the early Galactic life, nucleosynthesis was dominated by massive, 
short-living stars ending as type \textsc{ii} supernovae (SN), 
which produced $\alpha$-elements together with iron-peak elements.
Later, SN Ia resulting from the accretion of gas from a stellar companion onto a white dwarf also contributed to the enrichment of the interstellar medium, 
providing again iron-peak elements, but only little  amounts of $\alpha$-elements \citep[see \eg,][]{1979ApJ...229.1046T}.
As a result, metal-poor, old stars in the halo and thick disc show $\alpha$-elements enhancements with respect to younger, thin disc stars
(see the lecture by M. Haywood). There is a trend for $\alpha$-elements to increase 
when [Fe/H] increases with similar trends observed in disc, bulge, and halo
\citep{2010A&A...513A..35A}. 
The impact of $\alpha$-elements enhancements on stellar models is through opacity changes.
In the following, to estimate how the choice of $\alpha$-elements enhancement affects age-dating, 
we consider models with $\mathrm{[\alpha/Fe]}=0.0$ (\ie,  no enhancement with respect to the Sun) and $0.4$ dex 
(corresponding to the important enhancement observed in old population stars).


==> conclusion.tex <==
% ----------------------------------------------------------------
\begin{figure}[t]
\begin{center}
\resizebox{0.85\hsize}{!}{\includegraphics{FIGURES/hr_targets}}
\caption{ESTA-CoRoT comparisons. Evolutionary tracks in a HR diagram. 
Filled circles indicate the location of the stellar models (targets) chosen for the comparison.
Red lines correspond to the PMS, black lines to
the MS, and blue lines to the post MS evolution.
%The percentages indicate the larger relative age differences between the
%models from different evolutionary codes and the reference Cesam2k model.
[From \citet{2006ESASP1306..363M}.]}
\label{esta1}
\end{center}
\end{figure}
%-------------------------------------------------------------------

% ----------------------------------------------------------------
\begin{figure}[t]
\begin{center}
\resizebox{0.5\hsize}{!}{\includegraphics{FIGURES/glob_mean1_EES13}}\resizebox{0.5\hsize}{!}{\includegraphics{FIGURES/glob_max1_EES13}}
\caption{ESTA-CoRoT comparisons. {\sl Left:} mean differences in the classical parameters obtained in models
calculated with different codes and Cesam2k models. We distinguish in blue symbols the results of 
codes that have strictly
followed the prescription of the model calculation from the others in red  (see text).
{\sl Right:} same comparison showing the maximum differences obtained for each code.
[From  \citet{2010Ap&SS.328...29L}.]}
\label{esta2}
\end{center}
\end{figure}
%-------------------------------------------------------------------

The most appropriate method to obtain accurate stellar ages relies on the 
computation of stellar models. However these models are far from being perfect,
they are affected by several sources of uncertainties.
Some of them are well-known, some are difficult to identify. 
It is then not easy to provide ages with realistic error bars.  
With the nowadays, high-quality, ground and space data, efforts are made  to identify and 
quantify the  most important  biases affecting stellar age-dating. The ultimate goal is to eliminate them. 

In that respect, in the framework of the scientific preparation of the CoRoT mission, 
a European working group, ESTA-CoRoT, was in charge of carrying out in-depth comparisons of stellar models
\citep[see \eg,][]{2006ESASP1306..363M,2008Ap&SS.316....1L,2008ap&ss.316..187l,2008Ap&SS.316..219M}.  
The group has compared models calculated with ten different stellar evolutionary codes. 
Prescriptions had been given to have, as far as possible, the same input physics, physical constants, and astronomical constants 
in all codes. The model comparisons were made for several cases corresponding to different choices of the mass, 
initial chemical composition, and evolutionary stage \citep[for more details see][]{2006ESASP1306..363M,2008Ap&SS.316....1L}.
These cases were chosen to be representative of the CoRoT seismic targets.
The position in the HR diagram of one of the sets of models that have been compared is shown in Fig.~\ref{esta1}.
In Fig.~\ref{esta2} we show the comparisons of the radius, luminosity, effective temperature, and age
of the models calculated by each participating code with the results obtained with the Cesam2k code \citep{2008ap&ss.316...61m}. 
The left panel shows the mean relative differences in these quantities, while the right panel displays the
maximum differences. Concerning the age, the mean differences are in the range $1-12$ per cent, 
while the maximum differences
are in the range $2-43$ per cent, which is quite high. 
However, if we only consider the codes that strictly followed the prescriptions for the
comparison, that is adopting exactly the prescribed input physics and constants (blue symbols in Fig.~\ref{esta2}), 
the differences are reduced by a factor of about two. In this case, we can consider that 
the differences between the code results are only due to differences in numerical treatments, that is  
the handling of table interpolation (to get the opacity, EoS outputs, etc.),
the methods used to solve the equations, and hidden 
numerical mistreatments  
(time steps and mesh points, convective boundaries, etc.). The thorny problem of the numerical determination
of convective boundaries has been addressed recently by \citet{2014arXiv1405.0128G}.
More generally, numerical treatments are discussed in detail in \eg, \citet[][]{2008ap&ss.316..187l,2008Ap&SS.316..219M,2010Ap&SS.328...29L}, and references therein.

% ----------------------------------------------------------------
\begin{figure}[t]
\begin{center}
\resizebox{0.95\hsize}{!}{ \rotatebox{270}{\includegraphics{FIGURES/table_conclu_age}}}
%\resizebox{0.47\hsize}{!}{\includegraphics{Figs/fig_synth_2.eps}}
\caption{
%\orange{\sl Left:} 
Synthesis of the ranges of relative age differences at TO, as obtained when changing one of the inputs
of the  reference  model (defined in Sect.~\ref{grids}). 
From left to right, the case labels on the abscissae correspond to the following changes: 
[1, 2] [Fe/H] abundance by $\pm 0.1$ dex with respect to solar,
[3, 4]  initial helium abundance by $\pm 0.03$ with respect to solar,
[5] $\Delta Y/\Delta Z$ by $+3$ with respect to solar,
[6,7]  $\alpha$-elements enhancement of $+0.4$ dex at [Fe/H]=0.0 (a) and -1.0 dex (b),
[8] solar mixture ({\small AGSS09} vs. {\small GN93} mixture),
[9] opacity (increased by $10$ per cent),
[10] conductive opacity, \citet{1975ApJ...196..525I} vs. \citet{2007ApJ...661.1094C} formalism,
[11] $\sigma_{pp}$ reaction rate (decreased by $15$ per cent), 
[12, 13] $\sigma_\mathrm{CNO}$ (LUNA vs. NACRE rate for 
the $^{14}\mathrm{N} (p, \gamma) ^{15}\mathrm{O}$ rate) at [Fe/H]$=0.0$ dex (a) and $-2.0$ dex (c),
[14] screening factor in nuclear reaction rates (no screening vs. screening),
[15, 16]  atomic diffusion for (d) diffusion vs. no diffusion and (e) 
no diffusion vs. diffusion with diffusion velocities increased by $20$ per cent,
[17, 18] $\alpha_\mathrm{MLT}$ value by $\pm 0.20$ dex with respect to solar,
[19]  prescription for convection (MLT vs. FST), 
[20]  convective core overshooting ($\alpha_\mathrm{ov}=0.20$ vs. no overshooting),
[21, 22] rotation ($\Omega=50\ \mathrm{km.s^{-1}}$ vs. no rotation), at [Fe/H]=0.0 dex (a) and $\sim -1.0$ dex (b).
}
\label{synthesis}
\end{center}
\end{figure}
%-------------------------------------------------------------------

In the  present lecture, our approach has been to use the same evolutionary 
code (Cesam2k) to estimate
the impact of different physical inputs on the TO age value. 
The results are synthesized in Fig.~\ref{synthesis}, which highlights the huge impact of, on the one hand, the 
uncertain value of the initial helium abundance, and, on the other hand, the uncertain amount of mixing induced by overshooting  
and rotation, which determines the quantity of fuel available on the MS.
To better visualize the domain of mass and age concerned by model uncertainties, we show in 
Fig.~\ref{synthTO} the TO mass of observed stellar clusters of different ages, while in Fig.~\ref{synthmass} 
 we indicate the domain of mass associated to the different uncertainties in the model inputs.
We stress that the  model uncertainties do not add up linearly, 
 but correspond to the variation of one process at a time. Monte Carlo techniques can be used to 
estimate the cumulative effect  of all sources of uncertainties 
\citep[\eg,][]{1992ApJ...388..372C,2014A&A...561A.125V}.

% ----------------------------------------------------------------
\begin{figure}[t]
\begin{center}
\resizebox{0.90\hsize}{!}{\includegraphics{FIGURES/Mass_Age_TO_REF}}
\caption{
Value of the mass at turn-off as a function of age for
our reference models (solar [Fe/H]). The correspondence with observed stellar clusters
is indicated.
}
\label{synthTO}
\end{center}
\end{figure}
%-------------------------------------------------------------------
 
 % ----------------------------------------------------------------
 \begin{figure}[t]
 \begin{center}
 \resizebox{0.95\hsize}{!}{ \rotatebox{270}{\includegraphics{FIGURES/table_conclu_mass}}}
 \caption{
 The range of mass for which the age is affected by the different uncertainties in the model inputs considered here 
 (see Fig.~\ref{synthesis}). The effect of the chosen solar mixture is not reported because it affects the whole range of possible stellar
 masses.
 }
 \label{synthmass}
 \end{center}
 \end{figure}
 %-------------------------------------------------------------------
 
 
 
 %% ----------------------------------------------------------------
 \begin{figure}[h]
 \begin{center}
 \resizebox{0.5\hsize}{!}{\includegraphics{FIGURES/Gallart1}}\resizebox{0.5\hsize}{!}{\includegraphics{FIGURES/Gallart2}}
 %\resizebox{!}{0.5\vsize}{\includegraphics{Figs/Gallart1.png}}\resizebox{!}{0.5\vsize}{\includegraphics{Figs/Gallart2.png}}
 \caption{{\sl Left: } 
 tracks of $1.9 M_\odot$ models from two sets of grids (see text) plotted in the HR diagram together with 
 related isochrones providing the same TO location.
  {\sl Right:} three groups of isochrones
  providing the same TO and SGB position (same metallicity  $Z=0.001$).
  The  upper curves correspond to ages in the range $\sim  0.09-0.1$~\Gyr,
 the middle curves to ages in the range $\sim 0.4-0.8$~\Gyr, and the lower curves 
 correspond to ages in the range $\sim 2-3$~\Gyr. [Both figures from \citet{2005ARA&A..43..387G}.]
 }
 \label{conc5}
 \end{center}
 \end{figure}
 %-------------------------------------------------------------------
 
 Actually, different input physics are used in different stellar evolution codes. 
 As a result, different stellar ages are inferred from different grids of models. 
 \citet[][]{2005ARA&A..43..387G} compared evolution tracks of a $1.9\ M_\odot$ star in the HR diagram provided by
 the  BaSTI group \citep{2004apj...612..168p} and by the Padova group \citep{2002a&a...391..195g} and found that
 the same TO position is reached by isochrones of ages differing by 30 per cent (see Fig.~\ref{conc5}, left panel).
 This quite significant difference 
  is attributed to  several differences in the model inputs, in particular overshooting
  \citep{2004apj...612..168p}.
  \citet[][]{2005ARA&A..43..387G} also compared the ages of metal-deficient stellar populations that would be 
  predicted by different sets of model isochrones for three given choices of the pair (TO location, subgiant position).
  As shown in Fig.~\ref{conc5} {right panel}, the differences in age are more important for older stars: 
  at ages of ${\sim}0.1$~\Gyr~the predicted ages differ by ${\sim}10$ per cent, 
  while for older stars (ages of $0.4-0.8$ or $2-3$~\Gyr) the ages differ by $50-100$ per cent.
The differences are attributed to different model input physics 
 (atomic diffusion, overshooting, microscopic physics).
 
 To summarize, the present lecture showed that the physical description of stellar models  
 must still be significantly improved in
 order to provide accurate ages of MS stars at a precision level better than 20 per cent. 
 We could not discuss here all the processes which can affect the age determination.
 While the impact of numerics, input chemical composition, and microphysics can be estimated 
 rather easily, the impact of macrophysics is much more difficult to estimate because its description
 involves processes which are not well described, imply many parameters, 
 and are sometimes even unidentified.
 Furthermore, the present lecture focused on MS stars, therefore the sources of uncertainties
 on the time elapsed during advanced stages of stellar evolution have not been evaluated.
  
 Accurate ages at the level of 20 per cent or less for low mass MS stars are required in many
 astrophysical fields like the formation and evolution of planetary systems or the evolution of the Galaxy. 
 This need will be even more crucial when high-quality space data provided by, \eg, the 
 PLATO-ESA mission \citep{2013arxiv1310.0696r} and the Gaia-ESA mission \citep{2001a&a...369..339p}  will be available.
 Improving the physical description of stellar models is then certainly worth the effort.  
 The observational progress will have to be supported by theoretical and experimental developments, and by
 numerical simulations in 2-D and 3-D. For instance, recent progress came from the 
  the building of patched 1-D stellar models which include the convective outer layers obtained from 3-D simulations
  \citep{2012A&A...543A.120S}, and from 2-D rotating models such as those calculated with the ROTORC code \citep{1995ApJ...439..357D} and the 
  ESTER code  \citep{2013sf2a.conf..101R}.


==> convection.tex <==
\subsection{Convection}
\label{conv}

Heat and chemical element transport  by convection play an important role in
stellar evolution.  When integrating the  1D  equations for stellar structure, 
one only needs to determine where the medium is convective and how  
the temperature gradient is modified  in the convective regions 
and their surrounding layers. The way these pieces of information are obtained 
is described in all text books of stellar structure and evolution. 
We provide here a brief overview. %without detailing the derivations. 

 \subsubsection{Onset of convection }
  The onset of convection originates from a thermal
instability due to buoyancy. Convection takes place whenever 
the radiative gradient 
is not able  to transfer  the energy efficiently enough. 
Let us consider a gravitationally stratified medium with both temperature and density  
$T(z)$ and $\rho(z)$ decreasing outwards.  A blob 
 of gas, which is  slightly less dense (hotter) than the
surrounding medium, rises up from its equilibrium position  due to buoyancy. 
The Mach number  of the medium, $M_\mathrm{a}$, \ie,  
 the ratio of the convective velocity over the sound speed $v/c_\mathrm{s}$,  
 is small ($M_\mathrm{a} \sim 10^{-4}-0.3$ from the
 bottom to the top of the solar convective region). One then assumes  that pressure
equilibrium is maintained between the ascending bubble and its 
surroundings. Then at a given level, say $\delta r$,
above its initial position, the blob keeps on rising  
if it remains less dense than the surrounding medium (unstable
stratified medium). In contrast, gravity pulls the blob back if  
it becomes denser (cooler) than the surrounding environment 
(stably stratified medium, see Fig.~\ref{des1}). The rising blob 
(density $\rho^\prime$, temperature $T^\prime$)
remains less dense (hotter) {than} the cooling
medium ($\rho,T$) if the blob density decreases faster than that of the medium
 (its temperature decreases slower). This condition reads:
$$ \rho^\prime(r+\Delta r)< \rho(r+\Delta r)  \mathrm{\ \ or,\  equivalently\ \ }  T^\prime(r+\Delta r)> T(r+\Delta r). $$

 The condition for convective instability then is 
  $ \nabla^\prime < \nabla$ 
  with $\nabla=\mathrm{d}\log T/\mathrm{d}\log P$ for the medium and  $\nabla^\prime$ for  the blob. 

If the blob moves rapidly enough that its motion  can be assumed  adiabatic,  
$\nabla^\prime=\nabla_\mathrm{ad}=(\gamma-1)/\gamma$, 
where $\gamma=c_P/c_V$ is the ratio of the specific heat at constant pressure to the specific heat at
constant volume and $\gamma=5/3$ for an  ideal monoatomic gas. 
Then the condition for the onset of convection becomes
  $ \nabla_\mathrm{ad} < \nabla$. 

If the convection is inefficient,
 the temperature gradient of the medium 
remains nearly radiative hence $ \nabla \approx \nabla_\mathrm{rad}$. 
The reality lies in-between. The blob radiates energy during its motion, 
then $  \nabla^\prime>\nabla_\mathrm{ad} $. 
Convective heat transport decreases the temperature gradient of the medium,
 then $ \nabla < \nabla_\mathrm{rad}$. 
As a result,  the medium is usually characterized by 
\begin{equation} 
\label{gradall}
 \nabla_\mathrm{ad}<\nabla^\prime < \nabla  <\nabla_\mathrm{rad}.
 \end{equation}
The Schwarzschild criterion for convective instability in a homogeneous medium,  can
  then be conveniently stated as 
\begin{equation}\label{schwar}
 \nabla_\mathrm{ad}  <\nabla_\mathrm{rad}.
 \end{equation}
Both gradients are known at each level $r$,   
regions which are unstable against convection are then easily 
identified in 1-D stellar evolutionary codes, in the framework
of the mixing-length theory \citep{1932VeGoe...2..220B}.
%The determination of the
%extension of the associated chemically mixed region  is another story (see Sect.\ref{overshooting}). 
Furthermore, in presence of a $\mu$-gradient, the criterion for convective instability
becomes the Ledoux criterion \citep[\eg,][]{Kippenhahn13}.

%-----------------------------------------------
\begin{figure}
\begin{center}
\resizebox{0.85\hsize}{!}{\includegraphics{FIGURES/des1}}
\caption{Convective instability scheme.}
\label{des1}
\end{center}
\end{figure}
%-----------------------------------------------

 \subsubsection{Location of  convective regions in 1-D stellar models }

The next issue then is where in a stellar model the  criterion  for convective instability 
(Eq.~\ref{schwar}) is satisfied. Let us first consider the radiative gradient, 
$\nabla_\mathrm{rad}$ (defined in Eq.\ref{radiation}). It can also be written as 
$$\nabla_\mathrm{rad}= \frac{H_P}{KT} F_\mathrm{tot} \propto \kappa \frac{L}{m},$$ 
where $F_\mathrm{tot} $ is the total heat flux,  $H_P$ the pressure scale height, $L$ the
luminosity, and $K$ the thermal  conductivity, all at level $r$. 
In stars, convection can take place in the envelope, in the core, and in intermediate layers,
mainly because $\kappa$ or $L/m$ become large.

\begin{itemize}
\item {\sl Convective envelopes:} for a given star (with a given total luminosity  $L$
 and total mass $M$),  the opacity $\kappa$ in the envelope 
(where the mass $m$ at level $r$ is $m \sim M $) is large 
 due the presence of  $H^{-}$ ions in partial ionisation zones, hence the radiative gradient is large. 
Moreover, in these regions the value of $\gamma $ drops close to one  and therefore 
$\nabla_\mathrm{ad}$ becomes small. Both properties favour
the onset of convection.
  As a consequence, cool stars do develop
 extended  convective outer layers. The effective temperature, or the radius, depend on
 the properties of outer convection.
Hence uncertainties in the description of
inefficient convection in stellar models may affect the shape of the isochrones and 
 accordingly the ages deduced from isochrone fitting.

\item {\sl Convective  cores:} the ratio $L/m$  is quite large 
in the central regions 
when the nuclear energy rate strongly depends on
 temperature. This happens  when the CNO cycle  significantly operates, 
that is for MS stars of  
mass larger than about $1.1 ~ M_\odot$, depending on the
 chemical composition. 
Uncertainties in the location of the boundary of the central mixed region 
(see Sect.~\ref{overshooting})
involve variations of the lifetime of the central hydrogen burning phase and  
directly affect the ages. 
\end{itemize}

\subsubsection{Efficiency of convection }

The properties of stellar convection are governed by the competition 
between several characteristic time scales: \textsl{(i)} the buoyancy driving time scale 
$t_\mathrm{b}= 2 \pi/N_\mathrm{BV}$, where $N_\mathrm{BV}$, 
the Brunt-V\"{a}is\"{a}l\"{a}  (BV) frequency, 
is the frequency associated to the oscillation of a perturbed 
parcel of a gravitationally stratified fluid (see lecture 2), \textsl{(ii)} the viscous time scale 
$t_\mathrm{visc}=2 \pi/ \omega_{visc}$, 
and \textsl{(iii)} the radiative time scale $t_\mathrm{rad}=2 \pi/\omega_\mathrm{rad}$.
These latter quantities read,
\begin{equation}
\omega_\mathrm{visc}= \frac{\nu}{\ell^2} ~~~~~~;~~~~
\omega_\mathrm{rad}= \frac{K}{\ell^2}i \, ,
\end{equation}
where 
$\nu $ is the kinematic viscosity and $\ell$ a characteristic length scale.
The  Rayleigh number  measures the strength of the instability
$$ Ra = \frac{N_\mathrm{BV}^2}{\omega_\mathrm{visc}\; \omega_\mathrm{rad}} \; . $$
Both viscous and radiative effects inhibit the development of
 the instability.  In stellar conditions such as in the Sun, 
the Rayleigh number ($Ra_\mathrm{\odot} \sim 10^{23}$) is huge and the instability leads to 
a strong driving.
  
On the other hand, the Prandtl number of the 
fluid  measures the ratio of the thermal and viscous time scales:
$$ Pr = \frac{t_\mathrm{rad}}{t_\mathrm{visc}} = \frac{\omega_\mathrm{visc}}{\omega_\mathrm{rad}}.$$
In stellar conditions, $Pr$ is small ($Pr_\mathrm{\odot} \sim 10^{-10}-10^{-3}$) 
   and  the fluid can be considered as inviscid. 
As a consequence of the inviscid nature and of the
 large scales involved, the Reynolds number $Re$, is quite large. 
 With the characteristic length scale $L$,  say $L \sim 10^6-10^9$ m,
and velocity $U$, say  $U \sim 10^2-10^3 ~\mathrm{m \, s^{-1}}$,
the solar Reynolds number is  $$Re = \frac{UL}{\nu} \sim  10^{12}- 10^{14},$$ 
much larger than the critical number ($\approx~2300$) beyond which turbulence sets in.
Stellar convection is highly turbulent with a wide range 
of spatial scales involved  \citep[\eg,][]{2009LNP...756...49K}. %,2009LNP...756..107C}.

%($1\ \mathrm{Mm}$ - $1\ \mathrm{cm}$) 

As shown by 3-D simulations by \eg~\citet{1998ApJ...499..914S}, the
convective motions in stellar envelopes show  narrow 
cool descending plumes and hot rising bubbles, both types of motions penetrating
in the adjacent stably stratified layers. In 1-D stellar models, 
 however, the description of convection, the ``mixing length theory'' (MLT),  
 is based on  a very simple picture. It 
assumes that a blob which is less dense than the surrounding medium rises up  to a  level where 
it dissolves giving back its  energy excess to the
medium. The distance $d_\mathrm{MLT}$ is the mixing length 
and is usually taken as a fraction of the pressure scale height, $H_P$, that is 
  $d_\mathrm{MLT} = \alpha_\mathrm{MLT} \times H_P$. 

When convection takes place somewhere, its impact depends on its efficiency.  
 A measure of the efficiency $S$ is given by the ratio of the thermal time scale 
to the buoyancy time scale.
 $S$ is also the product of the Rayleigh number by the Prandtl number
\citep{1996apj...473..550c}. The quantity
\begin{equation}
\label{eff}
 S= \frac{t_\mathrm{rad}}{t_\mathrm{b}}\; = \; Ra \, \times \, Pr \; ,
 \end{equation}
measures the ability of convection to transport heat. 
The efficiency can then be either large or small. 
An inefficient convection $S\ll1$ however does not mean that the convective flux is small.
   
In stellar envelopes, convection is inefficient ($S\ll1$)
at the top of the convection zone. The
superadiabatic gradient defined as the difference between 
the actual gradient and the adiabatic 
one   is proportional to the squared mixing-length parameter: 
$$(\nabla-\nabla_\mathrm{ad})\propto \alpha_\mathrm{MLT}^2 $$

In convective cores, convection is quite efficient and the actual gradient is close to adiabatic
whatever the mixing-length value. On the other hand, non-local effects generate overshooting beyond the
Schwarzschild limit. This adds a new free parameter, the overshooting distance 
$d_\mathrm{ov}=\alpha_\mathrm{ov} \times H_P$. Therefore, the implementation of turbulent convective transport in  
1-D stellar codes  remains one major weak point of stellar
evolution theory.  Over the years, many tentative works  have aimed at extending the  phenomenological
description  proposed by \citet{1958za.....46..108b} after the work of 
\citet{1925Prandtl}. 
Despite these efforts, the MTL including its  improved variants (see below) 
 basically remains  in use in the current stellar evolutionary codes.
 
\subsubsection{Convective  gradient}
In stellar convective regions, one needs to determine the actual temperature gradient, $\nabla$. 
It is derived from the total flux conservation law 
  $F_\mathrm{tot}=F_\mathrm{rad} + F_\mathrm{conv}$, where the total
flux  is  known at each level $r$: 
$$F_\mathrm{tot}= \frac{L}{4\pi r^2} \; . $$
The radiative flux  depends on the unknown temperature gradient $$ F_\mathrm{rad}= -K ~ \nabla ~~~~;
~~~~K=\frac{4ac}{3}\frac{T^4}{\kappa \rho}\frac{1}{H_P} \; .$$
One also needs the convective flux $F_\mathrm{conv}$. Assuming pressure
equilibrium, the convective flux is identified with the enthalpy flux and is therefore 
  defined as $$ F_\mathrm{conv} = \rho~ c_p ~ <w~ \theta> \; , $$
where  
$\theta$ are the temperature deviations from the horizontal mean $T$, and $\omega$ the counterpart for
the vertical velocity. 
   Because of the turbulent nature of the convection, one must
 compute  an ensemble average of the statistical 
 fluctuations of velocity $w$ and temperature $\theta$
with respect to a static background. In order for turbulent convection implementation  to be tractable 
in a 1-D stellar code, several assumptions and approximations, listed belowr, have to be made.

\begin{itemize}
\item Convection can be assumed to be
incompressible because the Mach numbers are small ($Ma \ll1$).  
%The continuity equation  becomes $\nabla \cdot \vec v=0$. 
Actually, pressure and density fluctuations with respect to the averaged background 
are neglected except for the density fluctuation entering
the source of  convective instability, \ie,  the  buoyancy acceleration  $\delta \rho\times g$.

\item The second assumption is that of a stationary flow. 
All quantities are considered as statistical averages. 
This is justified by the fact that the dynamical time scales of
relevance for turbulent convection are much shorter than the evolutionary time
scale for MS stars.

\item The turbulence is assumed to be isotropic and homogeneous. 
The relevant quantities are horizontally averaged.  A better description 
ought to include the horizontal heat exchange between rising, hotter  blobs and cooler, descending plumes.  

\item  $\langle w \, \theta \rangle \; = \; {v} \, \Delta T$,  that is the product of  mean velocity times 
 mean temperature difference between the blob and the surrounding at the time of
 dissolution.
 
\item  Convection in 1-D stellar models is local, 
that is the convective gradient at a given level $r$ 
is written in terms of quantities defined at the same level. 
This is a strong assumption, which is
not justified. One consequence is a non-physical
treatment of the boundaries between radiative and
convective regions. They  are imposed
by the Schwarzschild criterion, which does not allow  for convective penetration into the
neighbouring radiative layers.

\item  The motion of the blob is assumed to stop  after some travel distance $l$ where 
it gives back  its heat excess to the medium. 
The distance is taken to be some fraction of $H_P$. 
This fraction is a free parameter, which
makes the formulation non predictable.  
In the solar case, this distance is derived from
a calibration process because the solar model must match its independently known mass, 
luminosity, and radius, at its current age. The value however depends on the physical inputs used
to build the solar model. There is no reason that the same value applies to another star with a
different mass, chemical composition, and age.  Actually, 3-D numerical simulations of
stellar envelopes show that the mixing length should vary across the HR diagram
 \citep[\eg,][]{2014arXiv1403.1062M}.
This is confirmed by seismic
studies of a few stars \citep[see \eg,][]{2005A&A...441..615M}.

\item   Turbulent pressure, turbulent kinetic energy are  discarded. 3-D simulations 
however show that they are not negligible \citep{1999A&A...351..689R,2003MNRAS.340..923R,2004IAUS..224..155T}.
\end{itemize}

With the above assumptions, using conservation of the flux and of the energy, 
it is possible to  derive a local relation between
the convective flux and the superadiatic gradient ($\nabla - \nabla_\mathrm{ad}$) such that 
$$F_\mathrm{conv}= -K_1 ~ (\nabla - \nabla_\mathrm{ad})  ~ \phi(S) \, , $$
where $\phi$ is a function of the efficiency $S$ (Eq.~\ref{eff}), 
and $K_1$ depends on the
equilibrium stratification properties.

In the formulation of \citet{1958za.....46..108b}, the heat is assumed to be  
transported by one eddy-size blobs (\ie, 
 corresponding to one single  spatial turbulent scale). 
Although this is an unjustified assumption, the resulting formulation 
 was and still is the one
implemented in  most 1-D stellar codes to compute the temperature gradient in regions of superadiabatic
(\ie,  inefficient) convection.
An improved formulation by \citet[][hereafter CM]{1991ApJ...370..295C} and \citet[][hereafter CGM]{1996apj...473..550c}  
takes into account the multi-spatial scale nature of stellar convection (Full Spectrum of Turbulence, FST). 
It has been implemented in a few stellar codes. As a result, the dependency of the  flux  on the efficiency, \ie,  the function 
$\phi(S)$, differs  between the two descriptions MLT and FST. 


%-----------------------------------------------
\begin{figure}
\begin{center}
\resizebox{0.85\hsize}{!}{\includegraphics{FIGURES/CM_S}}
\caption{The ratio of the efficiency dependency of the CGM
approach to that of the MLT as a function of the logarithm of the efficiency
$S$ (Eq.~\ref{eff}). After \citet{1996apj...473..550c}.
}
\label{CM_S}
\end{center}
\end{figure}
%-----------------------------------------------

Figure \ref{CM_S} from \citet{1996apj...473..550c} shows the ratio of the efficiency dependency of the CGM
approach to that of the MLT as a function of the logarithm of the efficiency $S$. 
The departure from one is the  consequence of including  the whole
 spectrum of kinetic energy in the FST convective flux. The plot   shows that 
the MLT underestimates the convective flux for high efficiency and overestimates
it for small efficiency. 

For an efficient convection ($S\gg1$) , one has:
$$\phi_\mathrm{CM} (S) \sim \phi_\mathrm{CGM} (S)  \sim 10\  \phi_\mathrm{MLT} (S)~;~~ F_\mathrm{conv}^\mathrm{CM} \gg F_\mathrm{conv}^\mathrm{MLT} \; .$$

For an inefficient convection, ($S\ll1$) 
$$\phi_\mathrm{CM} (S) \sim \frac{1}{3} ~\phi_\mathrm{CGM} (S)~~; ~~\phi_\mathrm{CGM} (S)\sim \frac{1}{3}~ \phi_\mathrm{MLT} (S)~~;~~ F_\mathrm{conv}^\mathrm{CM} \ll F_\mathrm{conv}^\mathrm{MLT} \; .$$

%Comparisons with 3D simulations show that the FST represents an improvement over the MLT 
%\citep{2008IAUS..252...75L,2007AIPC..948..141T}. 
Comparisons with  observations show that the FST represents an improvement over the MLT 
\citep{1995A&A...302..271G,1995A&A...302..382M}.
However it suffers from 
 the same other limitations as the MLT, 
particularly this is a local  theory which depends on a free parameter, the mixing length.

\subsubsection{Convection in stellar envelopes}

 In the MLT description, the efficiency is given by 
$$\Gamma \propto \alpha_\mathrm{MLT}~ \kappa ~ \Bigl(\frac{\rho}{T}\Bigr)^2, $$
where $\Gamma$ is  related to the efficiency $S$ as  $\Gamma \approx 0.025 ~ S$.
Because of the opacity peak in partial H ionization regions,  
near the superadiabatic layer (SAL), the opacity  $\kappa $ is   large.  
As a consequence, $(\nabla_\mathrm{rad}-\nabla_\mathrm{ad}) \gg1$ and the instability generates
 a strong driving. But $\rho / T$ is small in the outer
layers and  $\Gamma\ll1$ despite the strong driving. 
Convection is therefore inefficient in envelopes of cool stars.   
The temperature gradient then is intermediate between 
the radiative and the adiabatic gradient.  
For small efficiency, 
the gradient writes
 \begin{equation}
 \label{grad}
 \nabla \approx \nabla_\mathrm{rad}-\frac{9}{4}~ \Gamma^2 ~ (\nabla_\mathrm{rad}-\nabla_\mathrm{ad}) \; ,
 \end{equation}
see \eg~\citet{1958za.....46..108b,1992isa..book.....B}.
 The convective 
flux carries little energy
$$\frac{F_\mathrm{conv}}{F_\mathrm{tot}}\approx \frac{9}{4}~ \Gamma^2 ~
(1-\frac{\nabla_\mathrm{ad}}{\nabla_\mathrm{rad}}) \approx  \frac{9}{4}~ \Gamma^2 \ll1.$$  

%-----------------------------------------------
\begin{figure}
\begin{center}
\resizebox{0.5\hsize}{!}{\includegraphics{FIGURES/SAL_EES13_F29a}}\resizebox{0.5\hsize}{!}{\includegraphics{FIGURES/hr_EES13_F29b}}
\caption{ {\sl {\sl Left:}} profile of 
the superadiabatic gradient ($\nabla -\nabla_\mathrm{ad}$)
 as a function of  temperature $\log T$  in the  vicinity 
of the hydrogen ionisation region ($\log T\sim 4.1$)  in  a $1.0\  M_\odot$ model 
for two values of the
$\alpha_\mathrm{MLT}$ parameter,  $\alpha_\mathrm{MLT} = 0.7$ and  $\alpha_\mathrm{MLT}=1.8$. 
{\sl Right:}  HR diagram showing evolutionary tracks for two values of the mass 
and mixing-length parameter. 
The grey track corresponds to  $\alpha_\mathrm{MLT} = 0.7$ and the
black track is for $\alpha_\mathrm{MLT} =1.8$.
}
\label{sal}
\end{center}
\end{figure}
%-----------------------------------------------

\paragraph{Impact of the mixing-length value on the temperature gradient.} 
Left panel of Fig.~\ref{sal}  shows the  run of 
the superadiabatic gradient $(\nabla -\nabla_\mathrm{ad})$ 
 as a function of the temperature $T$ 
  in the  outer layers of a $1.0\ M_\odot$ model for two values of the
$\alpha_\mathrm{MLT}$ parameter  $\alpha_\mathrm{MLT} = 0.7$ and  $1.8$. 
From Eq.\ \ref{grad}, one obtains: 
$$ \nabla -\nabla_\mathrm{ad} \approx(1-\frac{9}{4}~ \Gamma^2) ~ (\nabla_\mathrm{rad}-\nabla_\mathrm{ad}).$$
For a given stratification, the mixing-length value determines the magnitude
 of the efficiency and therefore the gradient:
 the larger $\alpha_\mathrm{MLT}$, the larger the convective  efficiency and 
 the farther  the gradient from  the
 radiative one. The convective efficiency is small but the driving is strong 
$(\nabla_\mathrm{rad}-\nabla_\mathrm{ad})\gg1$ hence the  actual gradient in presence of convection 
is much larger than the adiabatic one  and closer to, although significantly
smaller than the radiative one.  How smaller depends on the value one adopts for
the mixing-length parameter. 

Below the SAL (up to $r/R =0.9 $, 
$\log  T =4.6$ for the $1.0\ M_\odot$ model), the convection becomes  quite efficient, \ie,  $\Gamma >1$, 
 because $\rho/T$ becomes  large.  For a large efficiency, one has
$$ \nabla \approx \nabla_\mathrm{ad} +\frac{9}{4 \Gamma} ~ (\nabla_\mathrm{rad}-\nabla_\mathrm{ad}) \sim \nabla_\mathrm{ad}.$$
The larger $\alpha_\mathrm{MLT}$, the larger the efficiency and the smaller the actual 
gradient compared to the radiative one, the closer to the adiabatic one.

\paragraph{Impact of the mixing-length value on evolutionary tracks.} The right panel of Fig.\ \ref{sal} 
shows the effect of  increasing $\alpha_\mathrm{MLT}$ on 
the evolutionary tracks in the HR diagram. The impact depends on the effective temperature, 
hence on the mass at a given luminosity. 
Stars of $T_\mathrm{eff}$ hotter than $\sim 7000 ~  K$ are not impacted 
 as can be seen for the $1.8 M_\odot$ tracks.  The reason is that the outer
  convection region is too thin and not dense enough 
   to play an important role in the energy transport. 

The comparison of the $1.0\ M_\odot$ tracks 
on the other hand shows that  there is a clear shift of the higher $\alpha_\mathrm{MLT}$ track 
toward the  blue for  models at the same
evolutionary stage, \ie,  with the same value of central hydrogen abundance.
For a larger $\alpha_\mathrm{MLT}$, the star is  more compact, 
the radius is smaller, and $T_\mathrm{eff}$ is higher  at  the same luminosity.
Hence, for low mass stars ($T_\mathrm{eff} <7000K$), an increase of $\alpha_\mathrm{MLT}$  causes
 an increase of $T_\mathrm{eff}$.

%-----------------------------------------------
\begin{figure}
\begin{center}
\resizebox{0.85\hsize}{!}{\includegraphics{FIGURES/diff_MLT_MLTm020_MLTp020}}
\caption{Same comparison as in Fig.~\ref{errorpp}. In blue the comparison of TO ages of the
reference model calculated with the 
solar $\alpha_\mathrm{MLT}=1.76$ value and a model calculated with
$\alpha_\mathrm{MLT}=\alpha_\mathrm{MLT,\odot}+0.20$. In red, the reference model 
is compared to a
model calculated with $\alpha_\mathrm{MLT}=\alpha_\mathrm{MLT,\odot}-0.20$.
}
\label{ageMLT}
\end{center}
\end{figure}
%-----------------------------------------------

\paragraph{Uncertainty on the mixing-length value: impact on TO ages.} 
Figure \ref{ageMLT} compares the age at TO of a reference model with solar composition
and solar $\alpha_\mathrm{MLT}$ value  with the TO ages of models 
 computed assuming   $\alpha_\mathrm{MLT,\odot}\pm 0.20$ dex.
The maximum effect of a change of $\alpha_\mathrm{MLT}$ by $\pm 0.20$ dex
 on the TO age occurs in the mass range  $1.2 -1.5\ M_\odot$. 
A maximum difference of 3 per cent is found at $1.4\ M_\odot$.
The impact is therefore small. The small impact on isochrones has been shown by
 \citet{1999MNRAS.303..265C}.

%-----------------------------------------------
\begin{figure}
\begin{center}
\resizebox{0.5\hsize}{!}{\includegraphics{FIGURES/hr_FST_MLT_EES13_F31}}\resizebox{0.5\hsize}{!}{\includegraphics{FIGURES/diff_REF_MLT}}
\caption{{\sl Left:} 
evolutionary  tracks  for $1.0\ M_\odot$  models computed assuming either 
 $\beta_\mathrm{CGM} =0.16$, 
 $\alpha_\mathrm{MLT} = 2.0 $, or $\alpha_\mathrm{MLT, \odot} = 1.76$ (all are solar calibrated values).
{\sl Right:} Same comparison as in Fig.~\ref{errorpp} between a model based on the MLT approach
(with $\alpha_\mathrm{MLT,\odot}=1.76$)
and a model based on the CGM approach (with $\alpha_\mathrm{CGM, \odot}=0.688$).
}
\label{FSTMLT}
\end{center}
\end{figure}
%-----------------------------------------------

\paragraph{FST versus MLT: impact on TO ages.}
As mentioned above, the FST theory provides an improved model of turbulent convection. That 
leads to a different prescription of the convective flux with respect 
to the standard MLT one. Nevertheless, the FST remains a local theory, which  
 also requires the definition of a mixing-length scale. Either 
$\Lambda_\mathrm{CGM}=z+\beta_\mathrm{CGM}\times H_{P,\mathrm{top}}$  
(where  $z$ is the distance to the convection boundary 
and $H_{P,\mathrm{top}}$ is the pressure scale-height at the top boundary), 
or $\Lambda_\mathrm{CGM}=\alpha_\mathrm{CGM}\times H_{P}$ are used. 
The free parameters $\beta_\mathrm{CGM}$, $\alpha_\mathrm{CGM}$, or  $\alpha_\mathrm{MLT}$  
are calibrated to fit the solar radius at solar age. 
Their values depend on the convective flux description, 
but also on input physics such as opacity, solar mixture, 
EoS, and atmospheric boundary conditions (BC), see \eg,  
\citet{1998A&A...332..127B,2004A&A...416.1081M,2006A&A...445..233S}.  
For instance, for a given set of microphysics and BC, we could match the current Sun with  either 
$\beta_\mathrm{CGM,\odot}=0.16$, $\alpha_\mathrm{CGM,\odot}=0.688$, or  $\alpha_\mathrm{MLT,\odot}=1.76$. 
However, because of the different dependence of the convective flux on the superadiabaticity, 
evolution
%For a calibrated Sun,  adopting the FST approach  instead of the MLT one 
% has a small effect  if one uses a \citet{1993ycat.6039....0k}'s
%model atmosphere; it is quite large if one uses an Eddington $T-\tau$ law
%\citep[e.g.][]{2002A&A...392..619H,2006A&A...445..233S,1999ApJ...526L..45K}. The evolution 
in the HR diagram with a constant $\alpha_\mathrm{MLT}$ value  is not equivalent 
to the evolution of a model of same mass with a constant value of $\alpha_\mathrm{CGM}$. 
As shown in left panel of Fig.\ref{FSTMLT}, while $\alpha_\mathrm{MLT} = 1.76$ 
yields a similar radius 
than CGM during the MS of a one solar mass model, its value must be increased to 
 $\alpha_\mathrm{MLT} = 2.0 $ during the RGB to mimic the same convective efficiency 
than the CGM treatment. 
 
%-----------------------------------------------
\begin{figure}
\begin{center}
\resizebox{0.45\hsize}{!}{\includegraphics{FIGURES/MLTisoc}}\resizebox{0.45\hsize}{!}{\includegraphics{FIGURES/Trampedach_hr}}
\caption{
{\sl Left:} isochrones calculated for the metallicity of the globular cluster M92. 
Continuous lines are for the FST treatment of convection and ages of $12$~\Gyr~ (left isochrone) and $14$~\Gyr~(right isochrone).
Dotted lines are isochrones of the same ages but calculated with the MLT treatment of convection.
Blue squares are observational data of M92 from \citet{1996PASP..108..560S}.  [From  
\citet{2001A&A...370..982M}.]  
{\sl Right:} variation of the $\alpha_\mathrm{MLT}$ value derived
from 3-D surface convection simulations  with a solar chemical composition 
in a $\log~ g - \log~ T_\mathrm{eff}$ diagram \citep{2011ApJ...731...78T}.
Evolutionary tracks with various masses are  from 
\citet{1992A&AS...96..269S,1999A&AS..135..405C}.
}
\label{MLTisocb}
\end{center}
\end{figure}
%-----------------------------------------------

A comparison assuming the solar calibrated values 
$\alpha_\mathrm{MLT,\odot}=1.76$ and $\alpha_\mathrm{CGM, \odot} =0.688$  (Fig.~\ref{FSTMLT}, right panel)
indicates that the impact on age at turn-off is small ($\Delta$age$/$age$ <3$ per cent). 
The maximum impact occurs for masses in the range $1.2-1.5 M_\odot$.
%for a solar composition with a maximum difference for 	a $1.4 M_\odot$ model. 
The impact on isochrones is small, for a constant  free parameter
 ($\alpha_\mathrm{MLT}$ or $\alpha_\mathrm{CGM}$). This remains  true for isochrones with low metallicity used to 
  reproduce  globular clusters. This is illustrated in Fig.~\ref{MLTisocb}, left panel, in the case of M92
 \citep[\eg,][]{1995A&A...302..382M,2001A&A...370..982M}. 

\paragraph{Calibrations of the mixing-length value.}  
 Figure \ref{MLTisocb} (right panel) shows the variation of the $\alpha_\mathrm{MLT}$ value derived
from 3-D surface convection simulations in a $\log~ g - \log~ T_\mathrm{eff}$ diagram
for evolutionary tracks of various masses  and a solar chemical
composition \citep{2011ApJ...731...78T}.  For a one solar mass for instance, the $\alpha_\mathrm{MLT}$  value 
roughly varies 
 from $1.8$ to $1.7$  on the MS. For  ZAMS models with masses decreasing from
 $1.$5 to $0.7\ M_\odot$, $\alpha_\mathrm{MLT}$ increases  from $1.7$ to $2.2$. 
  
One then needs to calibrate the $\alpha_\mathrm{MLT}$ value across the HR diagram. This can be obtained  
with a prescription  for the $\alpha_\mathrm{MLT}$ value derived from 2-D or
3-D numerical simulations 
\citep{1999A&A...346..111L,2008IAUS..252...75L,2011ApJ...731...78T,2014arXiv1403.1062M}. 
An alternative is 
to use patched models, which are built as  a 1-D stellar interior with the outer layers 
originating from a 3-D simulation 
\citep{1999A&A...351..689R,2006ApJ...636.1078S,2010A&A...509A..16S}.
An observational calibration  can also be directly
obtained on a case by case level by performing \`{a} la carte seismic studies (see lecture 2).


==> intro.tex <==
The age of stars cannot be obtained from direct measurements, it can only be estimated or inferred.
As reviewed by \citet{2010ara&a..48..581s}, many methods can be applied to age-date stars, depending on the mass and 
evolutionary stage of the star to be dated, and on whether the star is single or belongs to a group. There are three main 
categories of age-dating methods: quasi direct methods, stellar model dependent methods, and empirical methods. All  of them 
require at some level a knowledge of physical processes. These methods are discussed at different places in this
volume. To set the stage, we just briefly outline them in the following. Firstly, quasi-direct methods are based on 
nucleocosmochronometry, they are applied to the Sun (meteorite analysis, lecture by M. Gounelle at this
School, unpublished chapter) and to halo, very 
metal-poor stars (analyses of the lines of long-lived radio nuclides as Th or U, lecture by D. Valls-Gabaud).  Secondly, 
several empirical methods are currently used, as methods based on the decay of activity (measured from Ca~\textsc{ii} H and K, Mg~\textsc{ii}, 
and $\mathrm{H}\alpha$ lines or from the X-ray luminosity), on the decline of surface lithium abundance, or on the 
relation linking the rotation period and age (gyrochronology, see the lecture by R. Jeffries). 

Finally, several methods rely on stellar internal structure models. Single stars can be age-dated either through their placement on model isochrones 
(hereafter isochrone placement method, lecture by D. Valls-Gabaud) 
or through the fitting by stellar models of some particular stellar observable parameters (hereafter 
``\`{a} la carte'' method):
 
\begin{itemize}
\item \textbf{ Placement on model isochrones (or evolutionary tracks)} requires that, at least, indications of the 
star effective temperature $T_\mathrm{eff}$, luminosity $L$, and surface metallicity [Fe/H] are given by observations. This 
may require conversion from the colour-magnitude diagram to the theoretical Hertzsprung-Russell (HR) diagram (\eg, 
the lecture by S. Cassisi).  In this method, the theoretical isochrone that best matches the stellar observables 
provides the star age $A$, mass $M$, and initial metallicity. The method is widely used to age-date 
large samples of stars, either single or in clusters. For instance, it is applied to A-F stars of masses in the 
range $\approx 1.4- 2.5\ M_\odot$ in the Galactic discs, for Galactic evolution or populations studies and, to K-G 
metal-poor low-mass stars, in the halo or thick disc, for Galactic studies and cosmological applications. When stars belong 
to well-defined groups as open clusters, they can be assumed to be coeval and of the same initial chemical 
composition. In that case, particular features on the isochrones, sensitive to age, like the turn-off (TO) luminosity, are powerful 
tools to age-date the group. 
\item \textbf{\textsl{\`{A} la carte models}} are specific stellar models calculated to 
adjust the observational constraints of a given star, as the oscillation frequencies, interferometric radius, or, mass or radius if the star 
belongs to a binary system. \`{A} la carte models have to be calculated when precise ages are required, for instance to 
constrain the physical state of exoplanets or to better understand physical processes at work in stellar interiors (see Part 2 of these lectures in the chapter on \textsl{The impact of asteroseismology}).
\end{itemize}

In both methods, the accuracy on the inferred ages is impacted by the stellar model calculation 
procedure, in particular by the physical inputs or chemical composition of the models. Furthermore, 
empirical age-dating methods are also affected by stellar model uncertainties since they require calibrations, based on a physical 
knowledge of either stellar atmospheres, or stellar interiors and evolution. 
Other age-dating methods are lithium depletion boundary  which is almost model-independent, 
but only applicable to stars in coeval groups
(see the lecture by R. Jeffries), and the use of white dwarfs cooling sequences, a model-dependent method applicable to old stars (lecture by T. von Hippel).

In the present lectures, we focus on the precision and accuracy of age-dating based on the modeling of stellar interiors and evolution. 
More precisely, here in Lecture 1, we examine the main current uncertainties in the stellar model calculations 
and their impact on the age-dating process, while in lecture 2 we discuss the considerable improvement in age accuracy that results from asteroseismic analysis. 
The present Lecture 1 focuses on stars of masses in the range $0.6-40~M_\odot$, 
of both Population I and II, mainly on the main-sequence (MS). 
We evaluate the impact on age of the main inputs of stellar models (chemical composition, 
energy production, transport of energy and/or chemicals), 
focusing on the processes that have the most significant impact.
In Sect.~\ref{survey}, we recall some basics of stellar modeling and stellar age-dating.
Section~\ref{microphysics} discusses the impact of the chemical composition and of the microscopic input physics 
on the age of stellar models, while Sect.~\ref{macrophysics} examines the impact of the macrophysics.
In Sect.~\ref{conclusions} we provide a synthesis of the weights of the different 
stellar model uncertainties on the error on age.

